Numerical aspects of Casimir energy computation in acoustic scattering

Computing the Casimir force and energy between objects is a classical problem of quantum theory going back to the 1940s. Several different approaches have been developed in the literature often based on different physical principles. Most notably a representation of the Casimir energy in terms of determinants of boundary layer operators makes it accessible to a numerical approach. In this paper, we first give an overview of the various methods and discuss the connection to the Krein-spectral shift function and computational aspects. We propose variants of Krylov subspace methods for the computation of the Casimir energy for large-scale problems and demonstrate Casimir computations for several complex configurations. This allows for Casimir energy calculation for large-scale practical problems and significantly speeds up the computations in that case.

==> Spectral_properties.tex <==
{\color {blue} The matrix $M_{\infty}$ is a compact perturbation of matrix $M$, which makes the eigenvalues of them close to each other. Therefore, if we plot the eigenvalues of 
the matrix $MM_{\infty}^{-1}$, we can notice that there are many eigenvalues closed to 1 and nearly contributes nothing to the log determinant. This spectral property
inspires us to use some iteration method to approximate the extreme eigenvalues of $MM_{\infty}^{-1}$. In order to make the computation process more efficiently, 
we will introduce an inverse-free method to speed up this process which makes us deal with the large-scale problem in the future.}
